Where LLM Agents Fail and How They can Learn From Failures

Large Language Model (LLM) agents, which integrate planning, memory, reflection, and tool-use modules, have shown promise in solving complex, multi-step tasks. Yet their sophisticated architectures amplify vulnerability to cascading failures, where a single root-cause error propagates through subsequent decisions, leading to task failure. Current systems lack a framework that can comprehensively understand agent error in a modular and systemic way, and therefore fail to detect these errors accordingly. We address this gap with three contributions. First, we introduce the AgentErrorTaxonomy, a modular classification of failure modes spanning memory, reflection, planning, action, and system-level operations. Second, we construct AgentErrorBench, the first dataset of systematically annotated failure trajectories from ALFWorld, GAIA, and WebShop, grounding error analysis in real-world agent rollouts. Third, we propose AgentDebug, a debugging framework that isolates root-cause failures and provides corrective feedback, enabling agents to recover and iteratively improve. Experiments on AgentErrorBench show that AgentDebug achieves 24% higher all-correct accuracy and 17% higher step accuracy compared to the strongest baseline. Beyond detection, the targeted feedback generated by AgentDebug enables LLM agents to iteratively recover from failures, yielding up to 26% relative improvements in task success across ALFWorld, GAIA, and WebShop. These results establish principled debugging as a pathway to more reliable and adaptive LLM agents. The code and data will be available at https://github.com/ulab-uiuc/AgentDebug

==> content/XX-method-arch1.tex <==
We design \ModelName{} for agentic systems that operate over complete trajectories to produce: (i) comprehensive error detection across all steps and modules, and (ii) causal root-cause diagnosis with actionable feedback. The core principle is to identify the earliest critical decision whose correction would flip the trajectory from failure to success. This section describes our unified agent formulation, error taxonomy, and the two-stage debugging pipeline.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/method.pdf}
    \caption{\textbf{Overview of \ModelName{}.} (Left) Core modules—\emph{Planning}, \emph{Action}, \emph{Memory}, \emph{Reflection}—operate across varied environments. (Center) Unified rollout: Step~1 global plan, then plan$\rightarrow$act$\rightarrow$observe with memory/reflection updates. (Bottom) Failures are debugged into successes via actionable feedback, yielding paired traces. (Right) Training: Stage~1 step-level \emph{Error Detector}; Stage~2 global \emph{Root-Cause Analyzer} that pinpoints the earliest causal error and prescribes a fix.}

    \label{fig:method}
\end{figure}


\subsection{Error Detector Design}

Our debugging framework operates in two complementary stages: comprehensive error scanning followed by causal root-cause analysis. This design balances exhaustive detection with targeted intervention.

\paragraph{Stage 1: Comprehensive Error Detection}

Stage 1 functions as an error scanner that identifies all potential failures across the trajectory. For each step $t$, we detect the presence of error types from our taxonomy using a multi-label classifier:
$$p(\mathbf{y}_t \mid \tau_{\leq t}) = g_\theta(\text{Context}(s_{\leq t}, a_t, o_t))$$
where $\mathbf{y}_t \in \{0,1\}^K$ indicates $K$ error types. We implement $g_\theta$ as an instruction-tuned LLM (Qwen-8B/14B) prompted with the AET schema and few-shot examples. The model outputs structured predictions $(t, \mathcal{E}_t, \text{rationale}_t)$ containing detected errors and supporting evidence.

\paragraph{Stage 2: Causal Root-Cause Analysis}

While Stage 1 identifies where errors occur, Stage 2 determines which error caused the trajectory failure through causal reasoning. This distinction is crucial—many detected errors are symptoms rather than root causes.

\paragraph{Causal Criterion.} We identify the root cause as the earliest step whose correction would likely lead to task success. Formally, let $U(\tau) \in \{0,1\}$ indicate task success and $\mathsf{fix}_t(\tau)$ denote a minimal edit correcting step $t$'s error. We select:
$$t^* = \arg\min_t \; t \quad \text{s.t.} \quad \mathbb{P}[U(\mathsf{fix}_t(\tau)) = 1] \geq \gamma$$

This identifies the earliest intervention point with sufficient impact on the outcome.

\paragraph{Implementation.} Computing exact counterfactual probabilities is intractable. We implement root-cause analysis using GPT-4.1 as an LLM judge that performs causal reasoning over the complete trajectory. The judge takes as input the Stage 1 error detections $\{\mathcal{E}_t\}_{t=1}^T$ and the full trajectory $\tau$, then outputs a structured diagnosis:
$$\text{RootCause}(\tau, \{\mathcal{E}_t\}) \rightarrow \langle t^*, \text{error\_type}, \text{reasoning}, \text{feedback} \rangle$$

where $t^*$ identifies the critical step, $\text{error\_type} \in \text{AET}$ specifies the root-cause error category, $\text{reasoning}$ provides the causal chain analysis, and $\text{feedback}$ contains actionable correction instructions.

To optimize the LLM judge's accuracy, we conducted iterative refinement using our human-annotated validation set from AgentErrorBench. Through multiple rounds of prompt engineering and few-shot example curation, we improved the judge's performance in identifying true root causes versus superficial symptoms. The refinement process involved:
\begin{align}
\text{Judge}^{(k+1)} = \text{Refine}(\text{Judge}^{(k)}, \mathcal{V}_{\text{human}})
\end{align}

where each iteration incorporated failure cases from the previous round as additional few-shot examples and adjusted the causal reasoning instructions based on disagreements with human annotations. After five refinement iterations, our GPT-4.1 judge achieved 87\% accuracy in root-cause identification and 91\% agreement with human annotators on critical step selection, validated on a held-out test set of 100 expert-labeled trajectories.


\subsection{Inference}

Once the root cause $t^*$ is identified, \ModelName{} generates structured actionable feedback $\mathcal{F}_{t^*}$ containing four key components:
\begin{align}
\mathcal{F}_{t^*} = \langle \text{step}_{t^*}, \text{error\_type} \in \text{AET}, \text{correction}, \text{rationale} \rangle
\end{align}

where $\text{step}_{t^*}$ identifies the critical failure point, $\text{error\_type}$ specifies the categorized failure from our taxonomy, $\text{correction}$ provides a concrete fix (e.g., "Replace API call `search(query='hotels')` with `search(query='hotels', location='Paris')`"), and $\text{rationale}$ explains the causal chain (e.g., "The missing location parameter caused all subsequent hotel bookings to fail as they targeted wrong cities"). This feedback is designed to be interpretable and actionable, enabling agents to understand not just what went wrong, but why it matters for task completion.

The targeted intervention proceeds through localized re-rollout:
\begin{align}
\tau_{\text{new}} = \langle \tau_{<t^*}, \text{apply}(\mathcal{F}_{t^*}), \text{rollout}(s_{t^*}', \pi_{\text{corrected}}) \rangle
\end{align}

\paragraph{Iterative Debugging with Retry Budget.}
Recognizing that complex tasks may require multiple rounds of debugging, \ModelName{} supports iterative refinement with a retry budget $N$. The complete debugging loop operates as follows:
\begin{align}
\text{for } i = 1 \text{ to } N: \quad \tau^{(i)} = \begin{cases}
\tau^{(i-1)} & \text{if } U(\tau^{(i-1)}) = 1 \text{ (success)} \\
\text{Debug}(\tau^{(i-1)}) \rightarrow \tau_{\text{new}} & \text{if } U(\tau^{(i-1)}) = 0 \text{ (failure)}
\end{cases}
\end{align}

At each iteration, if the current trajectory fails, our error detector performs the two-stage analysis (comprehensive detection followed by root-cause identification), generates targeted feedback, and executes a localized re-rollout from the identified critical step. This process continues until either: (1) the task succeeds, or (2) the retry budget $N$ is exhausted. In practice, we find that $N=3$ strikes an effective balance between performance gains and computational cost, with most recoverable failures being resolved within 2 iterations. This iterative capability allows \ModelName{} to handle cascading failures where fixing one root cause may reveal another underlying issue, ultimately achieving up to 23\% improvement in task success rates compared to single-attempt baselines.


\paragraph{Iterative Debugging Pipeline.}
The complete \textbf{AgentDebug} pipeline iteratively applies the detect-diagnose-fix cycle up to $N$ times within a test-time compute budget. At each iteration $k$:
\begin{align}
\tau^{(k+1)} = \text{AgentDebug}(\tau^{(k)}) = \begin{cases}
\tau^{(k)} & \text{if } U(\tau^{(k)}) = 1 \\
\text{Rerun}(\tau^{(k)}, \mathcal{F}_{t^*}^{(k)}) & \text{otherwise}
\end{cases}
\end{align}


==> content/XX-method-arch2.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/method.pdf}
    \caption{\textbf{Overview of proposed \ModelName{}.} (Left) Normal rollouts cycle through memory, planning, reflection, and action. (Right) \ModelName{} debugs trajectories in three stages: (1) comprehensive scoring, (2) critical error detection, and (3) iterative re-rollouts with actionable feedback to flip failures into successes. }
    \label{fig:method}
\end{figure}

\begin{algorithm}[h]
\caption{\ModelName{} Framework with Agent Workflow}
\label{alg:model}
\begin{algorithmic}[1]
\Require Trajectory $\tau$, scoring functions $\{g_m\}$, budget $B$
\State Compute $\sigma_t^m=g_m(s_t,a_t)$, map to \AET{} error types $e_t^m$
\State Aggregate $\Sigma(\tau)=\tfrac{1}{T}\sum_t \sum_m w_m\sigma_t^m$
\If{$y(\tau)=1$} \Return $\tau$ \EndIf
\State $t^\ast \gets \arg\min_t \{ y(\tau^{(t \to \hat{a}_t)})=1 \}$
\State $\phi_{t^\ast}\gets\psi(s_{t^\ast},a_{t^\ast},e_{t^\ast})$
\For{$k=1$ to $B$}
    \State $\tau^{(k+1)}\gets\text{ReRollout}(\tau^{(k)},\phi_{t^\ast}^{(k)})$
    \If{$y(\tau^{(k+1)})=1$} \Return $\tau^{(k+1)}$ \EndIf
\EndFor
\State \Return Failure
\end{algorithmic}
\end{algorithm}



Given error analysis of agent failures, ideally we can develop an LLM with agentic workflow to refine LLM from failures.

We consider a generic agent formulation for the rollout agent which is prone to errors; then, we propose AgentDebug, a generic LLM that can fix the errors from the orignal rollout agent across different environments and rollout agent.
2

In low-resource academic setting, collecting a sufficient amount of data to potentially train an debug LLM will be cost prohibitive (est. cost XXX, with human labeling efforts). 
Instead, we developed an effective LLM workflow via prompt design that is cost efficient.
Note that our main purpose here is not to develop a SOTA debug LLM, instead, we aim to show that even with low-resource setting, our proposed TAXONOMY is highly effective in building a prompt based debug LLM workflow.

% \subsection{Trajectory Formulation}
\subsection{Key Modules of an LLM Agent}
We consider an agent $\pi$ interacting with an environment $\mathcal{E}$. A trajectory of length $T$ is:
\begin{equation}
    \tau = \{(s_1, a_1), (s_2, a_2), \dots, (s_T, a_T)\}, \quad s_t \in \mathcal{S},\; a_t \in \mathcal{A},
\end{equation}
where $\mathcal{S}$ and $\mathcal{A}$ denote the state and action spaces.  
Each action $a_t$ is generated through four modules:
\begin{equation}
    a_t = f_{\text{act}}\!\left(f_{\text{plan}}\!\left(f_{\text{refl}}\!\left(f_{\text{mem}}(s_t)\right)\right)\right),
\end{equation}
where $f_{\text{mem}}, f_{\text{plan}}, f_{\text{refl}}, f_{\text{act}}$ are the \textbf{Memory}, \textbf{Planning}, \textbf{Reflection}, and \textbf{Action} modules. We expect the agent may make errors in any the modules.

\subsection{\ModelName{} Framework}
\label{sec:modelname}

We design \ModelName{} as a debugging framework for single LLMs agent systems. As illustrated in Fig.~\ref{fig:method}, \ModelName{} explicitly analyzes full trajectories to:  
(i) assign comprehensive scores to every step and module,  
(ii) detect the earliest critical error, and  
(iii) guide re-rollouts with actionable feedback.  
The central principle is that correcting a single early decision can often flip the entire trajectory from failure to success.

As illustrated in Algorithm \ref{alg:model}, the inference procedure of \ModelName{} contains following stages:

\paragraph{Stage 1: Scoring with \AET{}.}  
We represent a trajectory $\tau=\{(s_1,a_1),\dots,(s_T,a_T)\}$ where each action is generated by  
\begin{equation}
    a_t = f_{\text{act}}(f_{\text{plan}}(f_{\text{refl}}(f_{\text{mem}}(s_t)))).
\end{equation}
Each module $m \in \{\text{mem},\text{plan},\text{refl},\text{act}\}$ is evaluated using  
\begin{equation}
    \sigma_t^m = g_m(s_t,a_t)\in[0,1],
\end{equation}
and combined into per-step and trajectory scores:  
\begin{equation}
    \sigma_t = \sum_m w_m\sigma_t^m, 
    \quad \Sigma(\tau)=\tfrac{1}{T}\sum_{t=1}^T\sigma_t.
\end{equation}
Importantly, each $\sigma_t^m$ is grounded in the \AET{} taxonomy, which maps steps to error types $e_t^m \in \mathcal{E}_{\text{err}}$ (e.g., planning constraint ignorance, action format error). This ensures that scoring is not only numeric but also interpretable in terms of root-cause categories.  

\paragraph{Stage 2: Critical Error Detection.}  
Let $y(\tau)\in\{0,1\}$ denote task outcome. We define the earliest critical step as  
\begin{equation}
    t^\ast = \arg\min_{t} \{\, y(\tau^{(t \to \hat{a}_t)})=1 \,\},
\end{equation}
where $\tau^{(t \to \hat{a}_t)}$ denotes a trajectory with corrected action $\hat{a}_t$. By linking $\hat{a}_t$ to the \AET{} error label $e_t^m$, \ModelName{} isolates not just \emph{when} the trajectory first goes wrong, but also \emph{why} (e.g., misrecall in memory, infeasible plan, or malformed action).  

\paragraph{Stage 3: Iterative Debugging.}  
For the detected error $e_{t^\ast}$, \ModelName{} generates targeted feedback
\begin{equation}
    \phi_{t^\ast} = \psi(s_{t^\ast},a_{t^\ast},e_{t^\ast}),
\end{equation}
and performs a re-rollout:
\begin{equation}
    \tau^{(k+1)} = \text{ReRollout}(\tau^{(k)},\phi_{t^\ast}^{(k)}), \quad k=1,\dots,B.
\end{equation}
The process repeats until $y(\tau^{(k+1)})=1$ or budget $B$ is reached. Theok feedback is conditioned on \AET{} categories, re-rollouts are interpretable and targeted rather than ad hoc.  




==> iclr2026/content/01-introduction.tex <==
% (1) Overall Correspondence of challenge 1, novelty 1, solution 1, ...
% (2) Q1: Think from demand: what are the attractive/necessary demands from the research community that have not been fully satisfied?
% (3) Q2: Relate to the community consensus/trend to show your importance. We point out the gap/potential/opportunities between the current consensus.
% (4) Q3: Crucial if you care about the impact and citations of your paper. Show your insights, help future researchers join our endeavor later. They will become your followers -- of your paper and yourself. These challenges are fundamental and have been tackled by your paper, but cannot be fully solved.
% (5) Q4: Prove your novelty: no one has solved XYZ, but we did. These limitations can be perfectly solved after your paper.
% (6) Q5: Solution XYZ to (partly) solve challenges and fill novelty gaps.

LLMs are increasingly capable of interacting with external environments, leveraging tools, and reasoning over memory, which enabled a new paradigm: LLMs Agents \citep{schick2023toolformer, qin2023toolllm, packer2023memgpt, shinn2023reflexion,liu2025advanceschallengesfoundationagents}. General purposed LLMs agents have driven advances across diverse domains, including embodied control, scientific discovery, open-ended web interaction, and research support \citep{zhou2023webarena, li2025metal, hong2025embodiedwebagentsbridging, zhu2025safescientistriskawarescientificdiscoveries}. Despite these achievements, current agents remain imperfect and insufficiently robust. They frequently exhibit errors—ranging from misinterpreting instructions and misusing tools to breaking down in long-horizon reasoning. These shortcomings underscore that, while promising, existing LLM Agents still lack the reliability required for real-world deployment. This observation motivates us to ask: \textit{\textbf{Where do LLM agents fail}} ?

While prior works have investigated the failures of LLM-based agents \citep{ji2024testing, sung2025verila, ning2024defining, cemri2025why, zhang2025which}, they have largely focused on enumerating error types or providing qualitative case studies. However, these analyses stop short of offering systematic mechanisms to trace failures back to their \textit{root causes}, and importantly, do not enable agents to fix these discovered failures based on such insights. To close this gap, we modularize error analysis with the explicit goal of tracing failures to their underlying causes. We conduct a large-scale study over hundreds of trajectories, decomposing each rollout into four operational modules: memory, reflection, planning, and action. By attributing each failure to its root module, we derive the \AET{} — a comprehensive taxonomy of failure modes designed to ground systematic error detection and guide the development of robust mitigation strategies. 

% Our highlights: modularize analysis that traces the root cause; 
% paradigm shift from offline error analysis to online error fix, crucial due to the dynamics and interactive environment: we move from purely offline error analysis, to an interface that allows debug agent to interact and fix the error only. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/teaser.pdf}
    \caption{\textbf{\textit{Motivation for \ModelName{}}}: A single root-cause failure (b) can propagate through subsequent steps (c), compounding errors and leading to task failure. \ModelName{} (d) addresses this bottleneck by tracing failures back to their source and providing actionable feedback that enables agents to evolve into more robust versions.}
    \label{fig:teaser}
    \vspace{-0.2in}
\end{figure}


%%% We identified the key bottleneck- Error Propagation
Our analysis reveals a critical bottleneck in LLM agents: \emph{error propagation}. As illustrated in Figure~\ref{fig:teaser}, a single root-cause failure (b) can cascade into successive errors (c), compounding degradation and leading to task failure. This challenge is especially acute in long-horizon tasks, where early mistakes distort later reasoning and actions, making recovery difficult. These insights motivate our central question: \textit{\textbf{How can LLM agents refine from failures}}?

%%% Prior works 
Recent progress in LLMs agent enhancement has largely centered on expanding the reasoning search space—through chain-of-thought~\citep{wei2023chainofthoughtpromptingelicitsreasoning}, tree-of-thought~\citep{yao2023treeofthoughts}, and graph-of-thought~\citep{besta2023graphofthoughts} approaches—or on incorporating step-level self-reflection \citep{yao2022react, yao2023treeofthoughts, besta2023graphofthoughts}, which allows agents to deliberate more thoroughly and locally revise their actions. While these advances improve flexibility and reasoning depth, they typically treat the trajectory as a sequence of isolated steps rather than as a coherent, interdependent process. 

% In reality, an agent’s trajectory is more akin to a program: it unfolds step by step, with dependencies, state changes, and side effects that accumulate over time. Viewing agents in this way suggests that improving their reliability is not only a modeling challenge but also an engineering one. Just as complex software systems require systematic debugging to trace and correct root-cause errors, agent systems demand principled debugging methodologies to enhance robustness. This perspective motivates us to propose debugging as the foundational mechanism for building more reliable LLM agents.


% summarize
% One of our key observations is that in reality, an agent’s trajectory is more akin to a program: it unfolds step by step, with dependencies, state changes, and side effects that accumulate over time. Viewing agents in this way suggests that improving their reliability is not only a modeling challenge but also an engineering one. Just as complex software systems require systematic debugging to trace and correct root-cause errors, agent systems demand principled debugging methodologies to enhance robustness. This perspective motivates us to propose debugging as the foundational mechanism for building more reliable LLM agents.

To address this challenge, we propose \ModelName{}, a debugging framework that decomposes a trajectory into decision steps, isolates the minimal set of root-cause failures, and provides corrective feedback back to the responsible states or actions. This process not only reduces noise from irrelevant errors but also highlights the key weaknesses that hinder successful task completion. As illustrated in Figure~\ref{fig:teaser} (d), \ModelName{} enables agents to iteratively evolve into more robust versions by learning directly from their failure cases. To rigorously evaluate whether models can detect critical errors and produce actionable feedback, we also construct the \Bench{}. This benchmark grounds the taxonomy in real-world trajectories, offering the first standardized testbed for error detection and debugging.

%%% Experiment summary
We evaluate \ModelName{} on \Bench{}, where it achieves 24\% higher all-correct accuracy (24.3\% vs. 0.3\%) and 17\% higher step accuracy (45.0\% vs. 28.0\%) compared to the strongest baseline. Beyond detection, the targeted feedback generated by \ModelName{} enables agents to iteratively recover from failures, yielding up to 26\% relative improvements in task success across ALFWorld, GAIA, and WebShop. Ablation studies further confirm that focusing on root-cause errors, rather than attempting to fix every surface-level mistake, is key to efficient debugging and meaningful performance gains.
%%%% Contribution
Overall, our contributions are summarized as follows:
\begin{itemize}[leftmargin=1.2em, itemsep=0.1em, topsep=0.25em]
    \item We analyze failed trajectories of LLM agents across diverse benchmarks and show that error propagation—early mistakes cascading into later failures—is the key bottleneck to robustness. From this study, we derive the \AET{}, a unified taxonomy of failure modes spanning planning, tool use, memory, and reflection.
    \item We introduce \Bench{}, the first curated dataset of systematically annotated failures from ALFWorld, GAIA, and WebShop. Each trajectory is labeled with fine-grained error categories and actionable feedback, providing a standardized testbed for studying, benchmarking, and comparing agent debugging methods.
    \item We present \ModelName{}, a debugging framework that identifies critical errors and provides actionable feedback. \ModelName{} achieves high root-cause detection accuracy, exceeding strong baselines by 24\%, and improves task success rates by 26\% across embodied reasoning, web interaction, and decision-making domains.
\end{itemize}


==> iclr2026/content/02-aet_bench.tex <==
To lay the foundation for our study of agent failures and debugging, this section introduces two \textit{proposed} components. Section~\ref{sub:aet} presents the \AET{}, a structured framework that organizes recurring failure modes into coherent modules. Section~\ref{sub:bench} then describes the \Bench{}, which grounds this taxonomy in systematically annotated trajectories from multiple environments. 

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{iclr2026/figures/aet_bench.pdf}
    \caption{\textbf{Pipeline of proposed \AET{} and \Bench{}}. Failed trajectories are collected, analyzed to develop a taxonomy of errors, and then annotated with root causes and actionable feedback to form the benchmark.}
    \label{fig:aet_bench_construction}
    \vspace{-0.2in}
\end{figure}

\subsection{Agent Failure Analysis}
\label{sub:aet}

To systematically investigate how agents fail, we collected over 500 failed trajectories from ALFWorld, WebShop, and GAIA, and conducted detailed human analyses to uncover recurring patterns. 
This study revealed the following central insight:

\begin{tcolorbox}[colback=berkeleyblue!5!white, colframe=berkeleyblue!100!black, boxrule=0.5mm, left=0.1mm, right=0.1mm, top=0.1mm, bottom=0.1mm]
\textbf{\textit{Key Insight.}} \textit{Error propagation is the primary bottleneck in LLM agent reliability.}  
Early mistakes rarely remain confined; instead, they cascade into subsequent steps, distorting reasoning, compounding misjudgments, and ultimately derailing the entire trajectory.
\end{tcolorbox}

Building on this insight, we introduce the \AET{}, a structured taxonomy that organizes recurring failure modes into five modules. Four capture the core operations of an agent—\textit{memory}, \textit{reflection}, \textit{planning}, and \textit{action}—while a fifth category accounts for \textit{system-level} errors that arise from external tools or infrastructure. This modular view not only enumerates common error types but also clarifies how weaknesses in one stage can cascade into others, enabling a principled approach to tracing and diagnosing failures.

\tcbset{
  colback=white,
  colframe=black!50,
  arc=4pt, % corner radius
  boxrule=0.5pt,
  left=2pt,
  right=2pt,
  top=2pt,
  bottom=2pt
}

\small
\begin{tcolorbox}
\begin{tabular}{>{\bfseries}m{0.18\linewidth} m{0.75\linewidth}}

\rowcolor{orange!10} \textit{Memory} & Errors in recalling or retrieving information (false recall, omission, retrieval failure) that distort subsequent reasoning. \\

\rowcolor{blue!10} \textit{Reflection} & Failures in monitoring progress or interpreting outcomes (progress misassessment, outcome misinterpretation), blocking course correction. \\

\rowcolor{green!10} \textit{Planning} & Logically unsound or infeasible strategies (impossible actions, constraint ignorance, incoherent subgoals) that cascade into missteps. \\

\rowcolor{yellow!15} \textit{Action} & Mistakes in executing operations (malformed outputs, incorrect parameters, missing arguments) that are visible but often mask upstream errors. \\

\rowcolor{red!15} \textit{System-level} & Failures outside reasoning, such as tool crashes, API mismatches, or exceeding step limits, highlighting system robustness issues. \\

\end{tabular}
\end{tcolorbox}

The \AET{} is designed not merely as a catalog of errors but as a causal lens for understanding how failures originate, propagate, and interact across modules. Full definitions are provided in Appendix~\ref{app:aet}.

\subsection{Agent Error Benchmark}
\label{sub:bench}

To rigorously evaluate whether models can detect critical errors and produce actionable feedback, we construct the \Bench{}. This benchmark grounds the taxonomy in real-world trajectories, offering the first standardized testbed for error detection and debugging.

The construction pipeline is shown in Figure~\ref{fig:aet_bench_construction}. We curated 200 representative trajectories: 100 from ALFWorld, 50 from WebShop, and 50 from GAIA. Ten expert annotators—graduate students with prior experience in NLP and LLMs agent research—labeled each trajectory using the \AET{} schema. Annotation proceeded at the decision-step level: every action, reflection, or plan was reviewed, and annotators tagged its error type(s) according to the taxonomy. In addition, they were tasked with identifying the minimal set of root-cause failures that explain the downstream error cascade, rather than exhaustively flagging all surface mistakes. This root-cause focus was emphasized through detailed guidelines and calibration examples, refined iteratively over three rounds of pilot annotation.

To ensure consistency, annotators first completed a training phase with feedback from the authors, followed by independent double-annotation on a shared subset of trajectories. Disagreements were adjudicated collectively, leading to several clarifications in category definitions (e.g., distinguishing “retrieval failure” under memory vs. “constraint ignorance” under planning). The final protocol balanced granularity with reliability, aiming for concise but causally meaningful tags. Inter-annotator agreement, measured using Cohen’s $\kappa$, reached $\kappa = \text{0.55}$ across modules, indicating substantial agreement.

The resulting dataset provides a quantitative view of how agents fail in practice. Figure~\ref{fig:failure_analysis} shows how errors emerge across steps, modules, and error types in the \Bench{}. It shows most failures cluster in mid-trajectory steps (6–15), where early missteps often cascade downstream. Memory and reflection dominate, with retrieval failures, hallucinations, and progress misjudgments leading to flawed planning. Action and system errors occur less frequently but remain critical, as malformed outputs or step-limit exhaustion can immediately terminate trajectories. The complete error type distribution is attached to Appendix \ref{app:failure_analysis}. 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.96\linewidth]{iclr2026/figures/Combined_Sankey.pdf}
    \caption{Distribution of failure cases in LLM agents on the \Bench{}}
    \label{fig:failure_analysis}
\end{figure}


Together, \AET{} and \Bench{} provide both the conceptual foundation and the empirical infrastructure for advancing robust LLM agents.


==> iclr2026/content/03-method.tex <==

% In low-resource academic setting, collecting a sufficient amount of data to potentially train an debug LLM will be cost prohibitive (est. cost XXX, with human labeling efforts). 
% Instead, we developed an effective LLM workflow via prompt design that is cost efficient.
% Note that our main purpose here is not to develop a SOTA debug LLM, instead, we aim to show that even with low-resource setting, our proposed TAXONOMY is highly effective in building a prompt based debug LLM workflow.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/method.pdf}
    \caption{\textbf{Overview of \ModelName{}.} (Left) LLM agent rollouts alternate between memory, planning, reflection, and action. (Right) \ModelName{} debugs trajectories in three stages: (1) fine-grained analysis across steps and modules, (2) detection of the critical error that triggers failure, and (3) iterative re-rollouts with actionable feedback to turn failures into successes.}
    \label{fig:method}
\end{figure}


% \begin{algorithm}[h]
% \small
% \DontPrintSemicolon
% \SetAlgoLined
% \LinesNotNumbered
% \KwIn{Trajectory $\tau = \{(s_t, a_t)\}_{t=1}^T$; Error taxonomy $\mathcal{E}_{\text{AET}}$; Max Iterations $I$}
% \KwOut{Corrected trajectory $\tau^*$ \textbf{or} \texttt{Failure}}

% \SetKwFunction{Eval}{Eval}
% \SetKwFunction{MapAET}{MapToAET}
% \SetKwFunction{Correct}{CorrectAction}
% \SetKwFunction{Replace}{ReplaceAction}
% \SetKwFunction{Reroll}{ReRollout}
% \SetKwFunction{GenFB}{GenFeedback}
% \SetKwFunction{UpdFB}{UpdateFeedback}

% \tcc{Stage 1: Fine-grained Analysis with AET}
% \For{$t \gets 1$ \KwTo $T$}{
%   \ForEach{$m \in \{\text{mem}, \text{plan}, \text{refl}, \text{act}\}$}{
%     $e_t^m \gets \MapAET(s_t,a_t,m,\mathcal{E}_{\text{AET}})$ \tcp*{Assign error type per module}
%   }
% }
% \If{\Eval{$\tau$} $=1$}{\Return $\tau$ \tcp*{Trajectory already successful}}

% \tcc{Stage 2: Critical Error Detection via Counterfactuals}
% $t^* \gets \varnothing$ \;
% \For{$t \gets 1$ \KwTo $T$}{
%   $\hat{a}_t \gets \Correct(s_t,a_t,\{e_t^m\}_{m})$ \tcp*{Generate corrected action}
%   $\hat{\tau} \gets \Replace(\tau,t,\hat{a}_t)$ \;
%   \If{\Eval{$\hat{\tau}$} $=1$}{
%     $t^* \gets t$ \tcp*{Earliest correction that removes final failure}
%     \textbf{break}
%   }
% }
% \If{$t^*=\varnothing$}{\Return \texttt{Failure} \tcp*{No critical error found}}

% \tcc{Stage 3: Iterative Debugging with Targeted Feedback}
% $\phi^{(0)} \gets \GenFB(s_{t^*},a_{t^*},\{e_{t^*}^m\}_{m})$ \tcp*{Actionable feedback}
% $\tau^{(0)} \gets \tau$ \;
% \For{$k \gets 1$ \KwTo $I$}{
%   $\tau^{(k)} \gets \Reroll(\tau^{(k-1)}, t^*, \phi^{(k-1)})$ \tcp*{Re-execute from $t^*$ with feedback}
%   \If{\Eval{$\tau^{(k)}$} $=1$}{\Return $\tau^{(k)}$}
%   $\phi^{(k)} \gets \UpdFB(\tau^{(k)}, \phi^{(k-1)})$ \tcp*{Refine guidance if still failing}
% }
% \Return \texttt{Failure} \tcp*{Max Attempts Reached}
% \caption{\ModelName{} Inference Procedure}
% \label{alg:model}
% \end{algorithm}

\begin{algorithm}[h]
\small
\DontPrintSemicolon
\SetAlgoLined
\LinesNotNumbered
\KwIn{Trajectory $\tau = \{(s_t, a_t)\}_{t=1}^T$; Error taxonomy $\mathcal{E}_{\text{AET}}$; Critical-error criterion $\mathcal{C}_{\text{crit}}$; Max Iterations $I$}
\KwOut{Corrected trajectory $\tau^*$ \textbf{or} \texttt{Failure}}

\SetKwFunction{Eval}{Eval}
\SetKwFunction{MapAET}{MapToAET}
\SetKwFunction{Reroll}{ReRollout}
\SetKwFunction{GenFB}{GenFeedback}
\SetKwFunction{UpdFB}{UpdateFeedback}
\SetKwFunction{Detect}{DetectCriticalErrors}

\tcc{Stage 1: Fine-grained Analysis with AET}
\For{$t \gets 1$ \KwTo $T$}{
  \ForEach{$m \in \{\text{mem}, \text{plan}, \text{refl}, \text{act}\}$}{
    $e_t^m \gets \MapAET(s_t,a_t,m,\mathcal{E}_{\text{AET}})$ \tcp*{Assign error type per module}
  }
}
\If{\Eval{$\tau$} $=1$}{\Return $\tau$ \tcp*{Trajectory already successful}}

\tcc{Stage 2: Critical Error Detection via LLM (no rollout/counterfactuals)}
$\mathcal{C} \gets \{\tau,\{e_t^m\}_{t,m},\mathcal{E}_{\text{AET}},\mathcal{C}_{\text{crit}}\}$ \tcp*{Pack analysis, taxonomy \& criterion}
$(\mathcal{T}^*, \mathcal{M}^*, \mathcal{Z}^*, \phi^{(0)}) \gets \Detect(\mathcal{C})$ \tcp*{LLM (fine-grained prompt)}
\If{$\mathcal{T}^*=\varnothing$}{\Return \texttt{Failure} \tcp*{No critical error found}}
$t^* \gets \min(\mathcal{T}^*)$ \tcp*{Earliest critical step}
\tcp{$\mathcal{T}^*$: set of critical steps; $\mathcal{M}^*$: modules per critical step; $\mathcal{Z}^*$: error-types per critical step}

\tcc{Stage 3: Iterative Debugging with Targeted Feedback}
$\tau^{(0)} \gets \tau$ \;
\For{$k \gets 1$ \KwTo $I$}{
  $\tau^{(k)} \gets \Reroll(\tau^{(k-1)}, t^*, \phi^{(k-1)})$ \tcp*{Re-execute from $t^*$ with feedback}
  \If{\Eval{$\tau^{(k)}$} $=1$}{\Return $\tau^{(k)}$}
  $\phi^{(k)} \gets \UpdFB(\tau^{(k)}, \phi^{(k-1)})$ \tcp*{Refine guidance if still failing}
}
\Return \texttt{Failure} \tcp*{Max Iterations Reached}
\caption{\ModelName{} Inference Procedure }
\label{alg:model}
\end{algorithm}


Building on our analysis of agent failures, we aim to develop method that actively refine themselves by learning from mistakes. We first formalize the key modules of an LLM-based agent in Section~\ref{sec:rollout}, and then present our proposed framework, \ModelName{}, in Section~\ref{sec:model}.


\subsection{Key Modules of an LLM Agent}
\label{sec:rollout}
As illustrated in Figure~\ref{fig:method}, we consider an agent that interacts with an environment over a sequence of steps.  
At each step, the agent observes a state and produces an action, forming a trajectory of state–action pairs.  
Each action is generated through four sequential modules: \textbf{Memory}, which recalls relevant past information; \textbf{Reflection}, which evaluates progress and interprets feedback; \textbf{Planning}, which formulates the next strategy; and \textbf{Action}, which executes the low-level operation.  
Errors can occur in any of these modules, and mistakes made early often propagate through later stages, compounding into larger failures.  This modular rollout design not only mirrors the agent’s internal decision process, but also provides a natural structure for human annotators to align errors with specific modules, making the diagnosis of agent failures more transparent and interpretable.  

\subsection{\ModelName{} Framework}
\label{sec:model}
We propose \ModelName{}, a debugging framework that enables single-LLM agents to diagnose and recover from their own failures across diverse environments. As illustrated in Fig.~\ref{fig:method}, \ModelName{} analyzes complete trajectories to (i) assign fine-grained error types to each step and module, (ii) identify the earliest critical error that directly causes the final failure, and (iii) provide actionable feedback to guide re-rollouts. The central intuition is that correcting a single root-cause mistake can often flip an otherwise failing trajectory into a successful one.

As presented in Algorithm~\ref{alg:model}, the inference procedure of \ModelName{} consists of three stages:

\paragraph{Stage 1: Fine-grained Analysis with \AET{}.}  
For each step in the trajectory, we analyze all four modules—memory, reflection, planning, and action.  
Each module is mapped to an \AET{} error type, grounding the analysis in interpretable categories such as “constraint ignorance” or “format error.”  
This produces a structured, module-level error profile for the trajectory.  

\paragraph{Stage 2: Critical Error Detection via Counterfactuals.}  
If the trajectory is already successful, no debugging is required.  
Otherwise, we perform counterfactual testing step by step: at each point, we substitute a corrected action and test whether the rollout would succeed.  
The \emph{critical error} is defined as the earliest step whose correction directly prevents the final failure.  
Unlike superficial mistakes or errors that are later corrected, the critical error is the root cause that truly determines whether the overall trajectory succeeds or fails—capturing both \emph{when} and \emph{why} the agent goes irreversibly off track.  

\paragraph{Stage 3: Iterative Debugging with Targeted Feedback.}  
Once the critical error is identified, the system generates feedback that specifies the error type and provides actionable guidance for refining subsequent actions and plans.  
The agent then re-executes (re-rolls out) the trajectory under this feedback. If the rollout still fails, the feedback is refined with more specific guidance, and the process repeats up to a fixed budget of attempts.  
Grounded in the \AET{} taxonomy, the feedback is both targeted and forward-looking—resolving the root cause while shaping how the agent approaches future steps.  





==> iclr2026/content/04-experiment.tex <==
\subsection{Critical Error Detection}
\label{subsec:rootcause}

\noindent{\textbf{Dataset.}}
We evaluate critical error localization on \Bench{} (Sec.~\ref{sub:bench}), which consists of 200 annotated failure trajectories.  
These trajectories are drawn from three representative benchmarks: \textbf{ALFWorld} \citep{shridhar2020alfworld}, \textbf{GAIA} \citep{mialon2023gaia}, and \textbf{WebShop} \citep{yao2022webshop}.  

\noindent{\textbf{Baselines.}}
We compare against three strategies: (1) \textbf{Direct Prompting}, which queries the LLM directly for error localization without any structured search; (2) \textbf{Brute Force}, which examines steps sequentially from $t{=}1$ to $T$, substituting a corrected action at each step and stopping once the rollout succeeds, thereby identifying the earliest critical step; and (3) \textbf{Binary Search}, which applies a divide-and-conquer procedure by probing the midpoint of the trajectory and recursively halving the search space until the critical step is isolated.  

\noindent{\textbf{Implementation.}}
We use GPT-4.1 as the base model, with the temperature set to 0 for deterministic outputs. The full prompt template is provided in the Appendix \ref{app:prompt}. 

\noindent{\textbf{Evaluation Metic.}} We evaluate critical error detection at multiple granularities, capturing both partial and complete localization ability. Specifically, we measure \textbf{Step} accuracy, the ability to identify the exact step where the first critical error occurs; %\textbf{Error Type} accuracy, the assignment of the correct fine-grained \AET{} label (e.g., constraint ignorance, format error); 
\textbf{Step+Module} accuracy, the joint prediction of both the correct step and its module; and \textbf{All Correct} (Step+Module+Error Type), a strict metric requiring the exact step, module, and error type to all be correctly identified.


\noindent{\textbf{Experiment Results}}  
Table~\ref{tab:exp1} shows that \ModelName{} consistently surpasses baselines across datasets and metrics. On average, \ModelName{} is 24\% more accurate in the All-Correct metric (24.3\% vs.\ 0.3\%) and improves Step accuracy by 61\% (45.0\% vs.\ 28.0\%). The gains are especially pronounced on GAIA, where Step accuracy nearly doubles (58.0\% vs.\ 30.0\%) and All-Correct triples (38.0\% vs.\ 12.0\%).

\begin{table}[hbtp]
\centering
\definecolor{GreenDark}{HTML}{34A853}
\definecolor{GreenLight}{HTML}{E6F4EA}
% 2. WebShop - 橙色系
\definecolor{OrangeDark}{HTML}{FBBC04}
\definecolor{OrangeLight}{HTML}{FEF8E7}
% 3. GAIA - 紫色系
\definecolor{PurpleDark}{HTML}{A142F4}
\definecolor{PurpleLight}{HTML}{F3E8FD}
% 4. Average - 粉色系
\definecolor{PinkDark}{HTML}{FF6D70}
\definecolor{PinkLight}{HTML}{FFEEEE}

\setlength{\tabcolsep}{6pt} % 调整列间距
\renewcommand{\arraystretch}{1.2} % 调整行高

\resizebox{\linewidth}{!}{\begin{tabular}{l ccc ccc ccc ccc}
\toprule
& \multicolumn{3}{c}{\cellcolor{GreenDark}\color{white}\textbf{ALFWorld}}
& \multicolumn{3}{c}{\cellcolor{OrangeDark}\color{white}\textbf{WebShop}}
& \multicolumn{3}{c}{\cellcolor{PurpleDark}\color{white}\textbf{GAIA}}
& \multicolumn{3}{c}{\cellcolor{PinkDark}\color{white}\textbf{Average}} \\

\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}

% --- 表头第二行：S, S+M, ALL ---
\textbf{Method}
& \cellcolor{GreenDark}\color{white}S & \cellcolor{GreenDark}\color{white}S+M & \cellcolor{GreenDark}\color{white}ALL
& \cellcolor{OrangeDark}\color{white}S & \cellcolor{OrangeDark}\color{white}S+M & \cellcolor{OrangeDark}\color{white}ALL
& \cellcolor{PurpleDark}\color{white}S & \cellcolor{PurpleDark}\color{white}S+M & \cellcolor{PurpleDark}\color{white}ALL
& \cellcolor{PinkDark}\color{white}S & \cellcolor{PinkDark}\color{white}S+M & \cellcolor{PinkDark}\color{white}ALL \\
\midrule

% --- 数据行：Baseline 方法 ---
Direct Prompting
& \cellcolor{GreenLight}28.0\% & \cellcolor{GreenLight}14.0\% & \cellcolor{GreenLight}1.0\%
& \cellcolor{OrangeLight}30.0\% & \cellcolor{OrangeLight}6.0\% & \cellcolor{OrangeLight}0.0\%
& \cellcolor{PurpleLight}26.0\% & \cellcolor{PurpleLight}10.0\% & \cellcolor{PurpleLight}0.0\%
& \cellcolor{PinkLight}28.0\% & \cellcolor{PinkLight}10.0\% & \cellcolor{PinkLight}0.3\% \\

Brute Force
& \cellcolor{GreenLight}10.0\% & \cellcolor{GreenLight}5.0\% & \cellcolor{GreenLight}0.0\%
& \cellcolor{OrangeLight}8.0\% & \cellcolor{OrangeLight}0.0\% & \cellcolor{OrangeLight}0.0\%
& \cellcolor{PurpleLight}18.0\% & \cellcolor{PurpleLight}8.0\% & \cellcolor{PurpleLight}0.0\%
& \cellcolor{PinkLight}12.0\% & \cellcolor{PinkLight}4.3\% & \cellcolor{PinkLight}0.0\% \\

Binary Search
& \cellcolor{GreenLight}20.0\% & \cellcolor{GreenLight}6.0\% & \cellcolor{GreenLight}1.0\%
& \cellcolor{OrangeLight}14.0\% & \cellcolor{OrangeLight}8.0\% & \cellcolor{OrangeLight}0.0\%
& \cellcolor{PurpleLight}22.0\% & \cellcolor{PurpleLight}10.0\% & \cellcolor{PurpleLight}0.0\%
& \cellcolor{PinkLight}18.7\% & \cellcolor{PinkLight}8.0\% & \cellcolor{PinkLight}0.3\% \\
\midrule

\textbf{\ModelName{}}
& \cellcolor{GreenLight}\textbf{35.0\%} & \cellcolor{GreenLight}\textbf{28.0\%} & \cellcolor{GreenLight}\textbf{21.0\%}
& \cellcolor{OrangeLight}\textbf{42.0\%} & \cellcolor{OrangeLight}\textbf{22.0\%} & \cellcolor{OrangeLight}\textbf{14.0\%}
& \cellcolor{PurpleLight}\textbf{58.0\%} & \cellcolor{PurpleLight}\textbf{44.0\%} & \cellcolor{PurpleLight}\textbf{38.0\%}
& \cellcolor{PinkLight}\textbf{45.0\%} & \cellcolor{PinkLight}\textbf{31.3\%} & \cellcolor{PinkLight}\textbf{24.3\%} \\

\bottomrule
\end{tabular}}
\caption{Comparison of methods across three environments (ALFWorld, WebShop, GAIA) and their average performance. Our method consistently outperforms baselines in all settings. Metrics shown are Step Exact (S), Step+Module (S+M), and All Correct (ALL).}
\label{tab:exp1}
\end{table}




% \begin{table}[htbp]
% \centering
% \small
% \renewcommand{\arraystretch}{1.0} % Adjust row spacing
% \setlength{\tabcolsep}{6pt} % Adjust column spacing
% \resizebox{\linewidth}{!}{
% \begin{tabular}{
%     l
%     |>{\columncolor{Color1}}c
%     |>{\columncolor{Color2}}c
%     |>{\columncolor{Color3}}c
%     |>{\columncolor{Color4}}c
%     |>{\columncolor{Color5}}c
%     |>{\columncolor{Color6}}c
% }
% \toprule
% \textbf{Method} & \textbf{Step} & \textbf{Step ($\pm$3)} & \textbf{Module} & \textbf{Error Type} & \textbf{Step+Module} & \textbf{All Correct} \\
% \midrule
% Direct Prompting & 12.5 & 65.0 & 50.0 & 25.0 & 12.5 & 7.5 \\
% Brute Force      & 10.0 & 55.0 & 32.5 & 15.0 & 2.5  & 2.5 \\
% Binary Search    & 5.0  & 25.0 & 15.0 & 10.0 & 0.0  & 0.0 \\
% \midrule
% Ours             & \textbf{50.0} & \textbf{85.0} & \textbf{65.0} & \textbf{50.0} & \textbf{45.0} & \textbf{42.5} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Critical Error Detection experiment results on \Bench{}.}
% \label{tab:detection}
% \end{table}





\subsection{Downstream Debugging on Single-Agent Benchmarks}
\label{subsec:downstream}

We next evaluate whether improved error detection leads to higher task success, testing if localizing root-cause failures enables agents to recover more effectively than baselines.

\noindent\textbf{Datasets.}  
Follow the previous experiment setting, we choose the evaluation data from three widely used single-agent benchmarks that cover complementary domains of reasoning and interaction: \textbf{ALFWorld} \citep{shridhar2020alfworld}, \textbf{GAIA} \citep{mialon2023gaia}, \textbf{WebShop} \citep{yao2022webshop}.

\noindent\textbf{Baselines.}  
We compare \textsc{AgentDebug} against several strong approaches. The first is Self-Refine, where the agent iteratively revises its outputs without explicit causal diagnosis of errors. The second is a Vanilla Debugger, which applies naive post-hoc corrections to failed trajectories without identifying the critical error taxonomy. Finally, we include strong test-time scaling baselines: Tree-of-Thought (ToT) and Best-of-$N$.  To ensure fairness, the max number of attempts of all baselines is matched to \textsc{AgentDebug} by total token usage, so any observed gains can be attributed to targeted error recovery rather than higher resource allocation.  

\noindent\textbf{Implementation.}  
We implement \textsc{AgentDebug} with up to $N=5$ re-rollouts, each beginning precisely at the identified critical step. This design enables the agent to explore alternative continuations directly from the point of failure rather than restarting from the beginning of the trajectory, thereby concentrating computational effort where it is most impactful. For backbone models of LLMs Agent, we evaluate across three representative systems of varying scales and architectures: GPT-4o-mini, Qwen3-8B, and Qwen3-Next-80B. 

\noindent\textbf{Experiment Results.} Figure~\ref{fig:experiment_4_2_1} reports the performance of \ModelName{} on the ALFWorld benchmark across three backbone LLM agents. On GPT-4o-mini, \ModelName{} boosts success from 21 (first attempt) to 55; on Qwen3-8B, from 48 to 74; and on Qwen3-Next-80B, from 60 to 84. These results show that \ModelName{} consistently outperforms all baselines and can effectively help LLM agents improve regardless of the backbone model, with especially large relative gains for smaller models. 


\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{iclr2026/figures/agent_tts_alfworld_comparison_tight.pdf}
    \caption{Downstream debugging performance on ALFWorld. Results are shown across three backbone models (GPT-4o-mini, Qwen3-8B, Qwen3-Next-80B) and differnt methods. \ModelName{} consistently outperforms strong baselines.}
    \label{fig:experiment_4_2_1}
\end{figure}

\begin{wrapfigure}{r}{0.40\textwidth}
    \vspace{-6pt} % tighten space above (tweak as needed)
    \centering
    \includegraphics[width=\linewidth]{iclr2026/figures/horizontal_comparison.pdf}
    \caption{Performance improvements comparison.}
    \label{fig:experiment_4_2_2}
    \vspace{-6pt} % tighten space below (tweak as needed)
\end{wrapfigure}


To further assess the generalizability of \ModelName{}, we move beyond ALFWorld and extend our evaluation to two additional benchmarks that stress complementary dimensions of agent reasoning: GAIA, which requires integrating open-domain knowledge and web-based tool use, and WebShop, which evaluates agents in a realistic e-commerce setting with structured constraints and transactional goals. Together, these benchmarks provide a diverse testbed spanning embodied interaction, knowledge-grounded reasoning, and goal-directed web navigation. Given the higher computational demands of these settings, we focus on comparing \ModelName{} against the two strongest baselines from our earlier experiments—Self-Refine and Best-of-$N$—which represent state-of-the-art approaches to iterative refinement and test-time scaling, respectively. The results, shown in Figure~\ref{fig:experiment_4_2_2}, demonstrate that \ModelName{} consistently delivers the largest gains across all three benchmarks. In particular, it achieves improvements of up to 26\% on ALFWorld and strong average performance on GAIA and WebShop, underscoring its robustness across diverse environments and confirming that targeted error detection and correction can outperform broader but less focused strategies such as scaling rollouts or unguided self-revision.


\begin{tcolorbox}[colback=californiagold!5!white, colframe=californiagold!100!black, boxrule=0.5mm, left=0.1mm, right=0.1mm, top=0.1mm, bottom=0.1mm]
\textbf{\textit{Findings}.} \ModelName{} consistently outperforms strong baselines in both error detection and downstream task success. Its ability to precisely localize root-cause failures (50.0\% step accuracy and 42.5\% all-correct accuracy) translates into substantial improvements in task performance, achieving up to 26\% relative gains across ALFWorld, GAIA, and WebShop. 
%These results highlight the effectiveness of principled debugging as a pathway toward more robust LLM agents.
\end{tcolorbox}


% \begin{tcolorbox}[colback=berkeleyblue!5!white, colframe=berkeleyblue!100!black, boxrule=0.5mm, left=0.1mm, right=0.1mm, top=0.1mm, bottom=0.1mm]
% \textbf{Takeaway.} ...
% \end{tcolorbox}



==> iclr2026/content/05-disscusion.tex <==
\subsection{Ablation Study}

% 1. Ablation on the debug step over three models on alfoworld test 100, gpt-4o-mini, qwen3-8b, qwen3-next-80b

% 2. Ablations on the different dection models

% 3. ablations on different rollout method:REACT REFLEXION, ACT ONLY, WITH MEMORY


To better understand the contribution of each component in our framework, we conduct a series of ablation studies. Specifically, we analyze the following factors.

\noindent{\textbf{Max Number of Attempts Allowed.}}  
We vary the maximum number of attempts of \ModelName{} with different base models— GPT-4o-mini, Qwen3-8B, and Qwen3-Next-80B—to examine how sensitive performance is to the chosen point of intervention. Results in Figure~\ref{fig:alfworld_success_rates} show that additional attempts yield consistent gains across all backbones, with especially pronounced improvements on smaller models such as GPT-4o-mini. This highlights the value of targeted re-rollouts in boosting task success.

\noindent{\textbf{\ModelName{} Base Models.}}  
We replace the base model of \ModelName{} with several alternatives to assess their impact on error localization and downstream success. As shown in Figure~\ref{tab:ablation_detector}, GPT-4.1 substantially outperforms other models, achieving 42\% step accuracy and 32\% strict all-correct accuracy. Competing base models such as Llama-3.3-70B, GPT-4o-mini, and Qwen3-Next-80B perform markedly worse.

\noindent{\textbf{Rollout Strategies.}}  
We compare several rollout paradigms—ReAct, Reflection, Act-only, and Memory+ReAct—against our proposed \textbf{Modular} strategy on Alfworld under the zero-shot setting. As shown in Table~\ref{tab:ablation_rollout}, \ModelName{}’s Modular rollout achieves the highest score (0.38), outperforming both reasoning-only and memory-augmented baselines. This result highlights the effectiveness of structured modularization is more reliably than alternative rollout designs.


\begin{figure}[htbp]
\centering

% --- Column 1: Plot ---
\begin{subfigure}{0.55\linewidth}
    \centering
    \includegraphics[width=\linewidth]{iclr2026/figures/task_success_rates_qwen_grouped.pdf}
    \caption{Success rates on Alfworld across five attempts.}
    \label{fig:alfworld_success_rates}
\end{subfigure}%
\hfill
% --- Column 2: Stacked Tables ---
\begin{subfigure}{0.45\linewidth}
    \centering
    
    % --- Subfigure B: Detector Table ---
    \begin{subfigure}{\linewidth}
        \centering
        \scriptsize
        \begin{tabular}{lcccc}
        \toprule
        \textbf{Base Model} & \textbf{Step} & \textbf{Error} & \textbf{Step+M} & \textbf{All} \\
        \midrule
        Llama-3.3-70B    & 16.0 & 16.0 & 6.0 & 2.0 \\
        GPT-4o-mini  & 14.0 & 10.0 & 4.0 & 2.0 \\
        Qwen3-Next-80B    &  4.0 & 14.0 & 2.0 & 2.0 \\
        \rowcolor{yellow!20}\textbf{GPT-4.1} & \textbf{42.0} & \textbf{44.0} & \textbf{32.0} & \textbf{32.0} \\
        \bottomrule
        \end{tabular}
        \caption{Base Model Performance Comparison.}
        \label{tab:ablation_detector}
    \end{subfigure}
    
    \vspace{0.5cm}
    
    % --- Subfigure C: Rollout Table (wider) ---
    \begin{subfigure}{1.1\linewidth} % make table C wider
        \centering
        \scriptsize
        \begin{tabular}{lc}
        \toprule
        \textbf{Rollout Strategy} & \textbf{Success Rate} \\
        \midrule
        Memory+ReAct & 0.34 \\
        Reflection   & 0.32 \\
        ReAct        & 0.26 \\
        Act Only     & 0.10 \\
        \rowcolor{yellow!20}\textbf{Modular} & \textbf{0.38} \\
        \bottomrule
        \end{tabular}

        \caption{Rollout Strategy Comparison.}
        \label{tab:ablation_rollout}
    \end{subfigure}
    
\end{subfigure}


\caption{Ablation study results. (a) Success rates on Alfworld, (b) comparison of detector models, and (c) rollout strategy analysis.}
\label{fig:ablation_combined}
\vspace{-0.1in}
\end{figure}

\subsection{Error Propagation}
\label{subsec:error_propoagate}

% Discussion over the error propagation, graphics and statistics
% some statistics by human and llm judge

% how often it cause the cascading effect(not always)

% how length it will cause the cascading effect

% which module and steps range cause the most of 

% some take away to prevent 

A key challenge in building robust LLM agents lies in understanding how small mistakes evolve into large-scale failures. Our analysis examines the phenomenon of error propagation—cases where an early misstep triggers a cascading effect that spreads throughout the trajectory. As shown in Figure \ref{fig:error_propagation},  early-stage mistakes cascade through later steps across tasks. The outlined cells indicate the first critical error in each trajectory, while progressively darker red shading reflects the compounding severity and persistence of errors over subsequent steps. This illustrates how initial failures frequently propagate forward, amplifying downstream task breakdowns.

\begin{figure}[ht]
    \centering
    \vspace{-8mm}
    \includegraphics[width=1\linewidth]{iclr2026/figures/grid_10x30_levels.pdf}
    \caption{\textbf{\textit{Illustration of Error Propagation}}: Darker shading indicating compounding failures and highlighting how initial mistakes amplify downstream breakdowns.}
    \vspace{-0.20in}
    \label{fig:error_propagation}
\end{figure}

Moreover, the likelihood and length of cascades vary significantly across modules. Memory and reflection errors are the most common sources of propagation, typically arising in early or mid-trajectory steps (around steps 5–15). Once an agent misremembers a fact or misjudges its progress, subsequent planning becomes systematically distorted, leading to repeated cycles of flawed action selection. Planning errors also contribute heavily, with constraint ignorance or infeasible strategies compounding as the agent attempts to execute them. By contrast, action-level errors are more visible and sometimes recoverable, though malformed outputs or missing parameters can still derail execution. System-level issues such as tool crashes or step-limit exhaustion act as immediate termination points rather than cascades.

These findings highlight two important takeaways for designing more reliable agents. First, \textbf{early detection and correction are critical}, since once cascades begin, they are difficult to reverse. Second, mechanisms that strengthen memory retrieval and reflection—such as external memory, progress tracking, or verification prompts—can substantially reduce the risk of propagation.




% \subsection{Case Study}
% sucessful debug case and how it can evolve through 

% one more specific error propagation case

% Statistics on the error types and steps distribution on benchmarks




==> iclr2026/content/06-related_works.tex <==

\paragraph{LLM-based Agentic Systems.}
Recent advances in LLM-based agents have demonstrated that combining planning, tool use, memory, and self-reflection can substantially improve performance on complex, multi-step tasks. The reasoning-acting paradigm, pioneered by ReAct \citep{yao2022react}, interleaves chain-of-thought reasoning with grounded environment actions. Test-time search methods such as Tree-of-Thoughts \citep{yao2023treeofthoughts} and Graph-of-Thoughts \citep{besta2023graphofthoughts} further expand the deliberation space through structured exploration. These systems are strengthened by external tool integration, ranging from self-supervised tool selection in Toolformer \citep{schick2023toolformer} to comprehensive tool ecosystems in ToolLLM \citep{qin2023toolllm}, as well as persistent memory mechanisms that maintain context across long horizons \citep{packer2023memgpt}. A critical aspect of robustness is the ability to reflect and self-correct: Reflexion \citep{shinn2023reflexion} introduces verbal self-reflection to revise future actions, while subsequent work explores richer feedback modalities and meta-cognitive strategies for deciding when to reflect versus act. Despite recent advances, the community still lacks a unified view of how agent components interact and fail. \ModelName{} fills this gap with a debugging layer that traces root causes across the plan–act–observe loop, detects failures from tool-use to memory, and generates corrective feedback that enables agents to improve through their mistakes.
\vspace{-0.1in}
\paragraph{Failure Analyses (Single- and Multi-Agent).}
Systematic failure analyses are emerging to quantify where agents break and how errors propagate. In multi-agent settings, recent works examine collaboration and competition dynamics~\citep{zhu2025multiagentbench}, role specialization, and emergent failure modes such as coordination collapse and dialogue drift \citep{cemri2025why,zhang2025which,zhu2025multiagentbench,hyun2025crewwildfire,tran2025multiagent}. For single-agent systems, analyses have highlighted planning brittleness, grounding and tool-use errors, and hallucination-induced cascades \citep{ji2024testing,sung2025verila,ning2024defining}. Compared to these studies, we focus on actionable debugging: moving from descriptive taxonomies to a two-stage detector that both identifies and helps fix root causes.
\vspace{-0.1in}
\paragraph{Test-Time Scaling for Agents.}
Scaling test-time compute improves reasoning and success rates by allocating more deliberation to challenging instances. In agents, this includes tree/graph search in thought space \citep{yao2023treeofthoughts,besta2023graphofthoughts}, best-of-$N$ sampling with self-consistency, and test-time compute scaling strategies \cite{li2025metal}. Our experiments position \ModelName{} orthogonally to compute scaling: even at fixed compute, targeted debugging recovers substantial performance, and when combined with scaling, it channels extra compute to the right failure points.

\vspace{-0.1in}

==> iclr2026/content/07-conclusion.tex <==
In summary, our work identifies error propagation as the central bottleneck to building robust LLM agents and introduces \AET{}, \Bench{}, and \ModelName{} as principled solutions. By tracing and correcting root-cause failures, \ModelName{} achieves substantial performance gains and establishes debugging as a foundation for agents that can continuously learn and evolve from their mistakes. While our work has limitations (see Appendix~\ref{app:limitation}), it paves the way toward more reliable and adaptive LLMs Agent.


==> iclr2026/content/XX-method-arch1.tex <==
We design \ModelName{} for agentic systems that operate over complete trajectories to produce: (i) comprehensive error detection across all steps and modules, and (ii) causal root-cause diagnosis with actionable feedback. The core principle is to identify the earliest critical decision whose correction would flip the trajectory from failure to success. This section describes our unified agent formulation, error taxonomy, and the two-stage debugging pipeline.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/method.pdf}
    \caption{\textbf{Overview of \ModelName{}.} (Left) Core modules—\emph{Planning}, \emph{Action}, \emph{Memory}, \emph{Reflection}—operate across varied environments. (Center) Unified rollout: Step~1 global plan, then plan$\rightarrow$act$\rightarrow$observe with memory/reflection updates. (Bottom) Failures are debugged into successes via actionable feedback, yielding paired traces. (Right) Training: Stage~1 step-level \emph{Error Detector}; Stage~2 global \emph{Root-Cause Analyzer} that pinpoints the earliest causal error and prescribes a fix.}

    \label{fig:method}
\end{figure}


\subsection{Error Detector Design}

Our debugging framework operates in two complementary stages: comprehensive error scanning followed by causal root-cause analysis. This design balances exhaustive detection with targeted intervention.

\paragraph{Stage 1: Comprehensive Error Detection}

Stage 1 functions as an error scanner that identifies all potential failures across the trajectory. For each step $t$, we detect the presence of error types from our taxonomy using a multi-label classifier:
$$p(\mathbf{y}_t \mid \tau_{\leq t}) = g_\theta(\text{Context}(s_{\leq t}, a_t, o_t))$$
where $\mathbf{y}_t \in \{0,1\}^K$ indicates $K$ error types. We implement $g_\theta$ as an instruction-tuned LLM (Qwen-8B/14B) prompted with the AET schema and few-shot examples. The model outputs structured predictions $(t, \mathcal{E}_t, \text{rationale}_t)$ containing detected errors and supporting evidence.

\paragraph{Stage 2: Causal Root-Cause Analysis}

While Stage 1 identifies where errors occur, Stage 2 determines which error caused the trajectory failure through causal reasoning. This distinction is crucial—many detected errors are symptoms rather than root causes.

\paragraph{Causal Criterion.} We identify the root cause as the earliest step whose correction would likely lead to task success. Formally, let $U(\tau) \in \{0,1\}$ indicate task success and $\mathsf{fix}_t(\tau)$ denote a minimal edit correcting step $t$'s error. We select:
$$t^* = \arg\min_t \; t \quad \text{s.t.} \quad \mathbb{P}[U(\mathsf{fix}_t(\tau)) = 1] \geq \gamma$$

This identifies the earliest intervention point with sufficient impact on the outcome.

\paragraph{Implementation.} Computing exact counterfactual probabilities is intractable. We implement root-cause analysis using GPT-4.1 as an LLM judge that performs causal reasoning over the complete trajectory. The judge takes as input the Stage 1 error detections $\{\mathcal{E}_t\}_{t=1}^T$ and the full trajectory $\tau$, then outputs a structured diagnosis:
$$\text{RootCause}(\tau, \{\mathcal{E}_t\}) \rightarrow \langle t^*, \text{error\_type}, \text{reasoning}, \text{feedback} \rangle$$

where $t^*$ identifies the critical step, $\text{error\_type} \in \text{AET}$ specifies the root-cause error category, $\text{reasoning}$ provides the causal chain analysis, and $\text{feedback}$ contains actionable correction instructions.

To optimize the LLM judge's accuracy, we conducted iterative refinement using our human-annotated validation set from AgentErrorBench. Through multiple rounds of prompt engineering and few-shot example curation, we improved the judge's performance in identifying true root causes versus superficial symptoms. The refinement process involved:
\begin{align}
\text{Judge}^{(k+1)} = \text{Refine}(\text{Judge}^{(k)}, \mathcal{V}_{\text{human}})
\end{align}

where each iteration incorporated failure cases from the previous round as additional few-shot examples and adjusted the causal reasoning instructions based on disagreements with human annotations. After five refinement iterations, our GPT-4.1 judge achieved 87\% accuracy in root-cause identification and 91\% agreement with human annotators on critical step selection, validated on a held-out test set of 100 expert-labeled trajectories.


\subsection{Inference}

Once the root cause $t^*$ is identified, \ModelName{} generates structured actionable feedback $\mathcal{F}_{t^*}$ containing four key components:
\begin{align}
\mathcal{F}_{t^*} = \langle \text{step}_{t^*}, \text{error\_type} \in \text{AET}, \text{correction}, \text{rationale} \rangle
\end{align}

where $\text{step}_{t^*}$ identifies the critical failure point, $\text{error\_type}$ specifies the categorized failure from our taxonomy, $\text{correction}$ provides a concrete fix (e.g., "Replace API call `search(query='hotels')` with `search(query='hotels', location='Paris')`"), and $\text{rationale}$ explains the causal chain (e.g., "The missing location parameter caused all subsequent hotel bookings to fail as they targeted wrong cities"). This feedback is designed to be interpretable and actionable, enabling agents to understand not just what went wrong, but why it matters for task completion.

The targeted intervention proceeds through localized re-rollout:
\begin{align}
\tau_{\text{new}} = \langle \tau_{<t^*}, \text{apply}(\mathcal{F}_{t^*}), \text{rollout}(s_{t^*}', \pi_{\text{corrected}}) \rangle
\end{align}

\paragraph{Iterative Debugging with Retry Budget.}
Recognizing that complex tasks may require multiple rounds of debugging, \ModelName{} supports iterative refinement with a retry budget $N$. The complete debugging loop operates as follows:
\begin{align}
\text{for } i = 1 \text{ to } N: \quad \tau^{(i)} = \begin{cases}
\tau^{(i-1)} & \text{if } U(\tau^{(i-1)}) = 1 \text{ (success)} \\
\text{Debug}(\tau^{(i-1)}) \rightarrow \tau_{\text{new}} & \text{if } U(\tau^{(i-1)}) = 0 \text{ (failure)}
\end{cases}
\end{align}

At each iteration, if the current trajectory fails, our error detector performs the two-stage analysis (comprehensive detection followed by root-cause identification), generates targeted feedback, and executes a localized re-rollout from the identified critical step. This process continues until either: (1) the task succeeds, or (2) the retry budget $N$ is exhausted. In practice, we find that $N=3$ strikes an effective balance between performance gains and computational cost, with most recoverable failures being resolved within 2 iterations. This iterative capability allows \ModelName{} to handle cascading failures where fixing one root cause may reveal another underlying issue, ultimately achieving up to 23\% improvement in task success rates compared to single-attempt baselines.


\paragraph{Iterative Debugging Pipeline.}
The complete \textbf{AgentDebug} pipeline iteratively applies the detect-diagnose-fix cycle up to $N$ times within a test-time compute budget. At each iteration $k$:
\begin{align}
\tau^{(k+1)} = \text{AgentDebug}(\tau^{(k)}) = \begin{cases}
\tau^{(k)} & \text{if } U(\tau^{(k)}) = 1 \\
\text{Rerun}(\tau^{(k)}, \mathcal{F}_{t^*}^{(k)}) & \text{otherwise}
\end{cases}
\end{align}


==> iclr2026/content/XX-method-arch2.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{figures/method.pdf}
    \caption{\textbf{Overview of proposed \ModelName{}.} (Left) Normal rollouts cycle through memory, planning, reflection, and action. (Right) \ModelName{} debugs trajectories in three stages: (1) comprehensive scoring, (2) critical error detection, and (3) iterative re-rollouts with actionable feedback to flip failures into successes. }
    \label{fig:method}
\end{figure}

\begin{algorithm}[h]
\caption{\ModelName{} Framework with Agent Workflow}
\label{alg:model}
\begin{algorithmic}[1]
\Require Trajectory $\tau$, scoring functions $\{g_m\}$, budget $B$
\State Compute $\sigma_t^m=g_m(s_t,a_t)$, map to \AET{} error types $e_t^m$
\State Aggregate $\Sigma(\tau)=\tfrac{1}{T}\sum_t \sum_m w_m\sigma_t^m$
\If{$y(\tau)=1$} \Return $\tau$ \EndIf
\State $t^\ast \gets \arg\min_t \{ y(\tau^{(t \to \hat{a}_t)})=1 \}$
\State $\phi_{t^\ast}\gets\psi(s_{t^\ast},a_{t^\ast},e_{t^\ast})$
\For{$k=1$ to $B$}
    \State $\tau^{(k+1)}\gets\text{ReRollout}(\tau^{(k)},\phi_{t^\ast}^{(k)})$
    \If{$y(\tau^{(k+1)})=1$} \Return $\tau^{(k+1)}$ \EndIf
\EndFor
\State \Return Failure
\end{algorithmic}
\end{algorithm}



Given error analysis of agent failures, ideally we can develop an LLM with agentic workflow to refine LLM from failures.

We consider a generic agent formulation for the rollout agent which is prone to errors; then, we propose AgentDebug, a generic LLM that can fix the errors from the orignal rollout agent across different environments and rollout agent.
2

In low-resource academic setting, collecting a sufficient amount of data to potentially train an debug LLM will be cost prohibitive (est. cost XXX, with human labeling efforts). 
Instead, we developed an effective LLM workflow via prompt design that is cost efficient.
Note that our main purpose here is not to develop a SOTA debug LLM, instead, we aim to show that even with low-resource setting, our proposed TAXONOMY is highly effective in building a prompt based debug LLM workflow.

% \subsection{Trajectory Formulation}
\subsection{Key Modules of an LLM Agent}
We consider an agent $\pi$ interacting with an environment $\mathcal{E}$. A trajectory of length $T$ is:
\begin{equation}
    \tau = \{(s_1, a_1), (s_2, a_2), \dots, (s_T, a_T)\}, \quad s_t \in \mathcal{S},\; a_t \in \mathcal{A},
\end{equation}
where $\mathcal{S}$ and $\mathcal{A}$ denote the state and action spaces.  
Each action $a_t$ is generated through four modules:
\begin{equation}
    a_t = f_{\text{act}}\!\left(f_{\text{plan}}\!\left(f_{\text{refl}}\!\left(f_{\text{mem}}(s_t)\right)\right)\right),
\end{equation}
where $f_{\text{mem}}, f_{\text{plan}}, f_{\text{refl}}, f_{\text{act}}$ are the \textbf{Memory}, \textbf{Planning}, \textbf{Reflection}, and \textbf{Action} modules. We expect the agent may make errors in any the modules.

\subsection{\ModelName{} Framework}
\label{sec:modelname}

We design \ModelName{} as a debugging framework for single LLMs agent systems. As illustrated in Fig.~\ref{fig:method}, \ModelName{} explicitly analyzes full trajectories to:  
(i) assign comprehensive scores to every step and module,  
(ii) detect the earliest critical error, and  
(iii) guide re-rollouts with actionable feedback.  
The central principle is that correcting a single early decision can often flip the entire trajectory from failure to success.

As illustrated in Algorithm \ref{alg:model}, the inference procedure of \ModelName{} contains following stages:

\paragraph{Stage 1: Scoring with \AET{}.}  
We represent a trajectory $\tau=\{(s_1,a_1),\dots,(s_T,a_T)\}$ where each action is generated by  
\begin{equation}
    a_t = f_{\text{act}}(f_{\text{plan}}(f_{\text{refl}}(f_{\text{mem}}(s_t)))).
\end{equation}
Each module $m \in \{\text{mem},\text{plan},\text{refl},\text{act}\}$ is evaluated using  
\begin{equation}
    \sigma_t^m = g_m(s_t,a_t)\in[0,1],
\end{equation}
and combined into per-step and trajectory scores:  
\begin{equation}
    \sigma_t = \sum_m w_m\sigma_t^m, 
    \quad \Sigma(\tau)=\tfrac{1}{T}\sum_{t=1}^T\sigma_t.
\end{equation}
Importantly, each $\sigma_t^m$ is grounded in the \AET{} taxonomy, which maps steps to error types $e_t^m \in \mathcal{E}_{\text{err}}$ (e.g., planning constraint ignorance, action format error). This ensures that scoring is not only numeric but also interpretable in terms of root-cause categories.  

\paragraph{Stage 2: Critical Error Detection.}  
Let $y(\tau)\in\{0,1\}$ denote task outcome. We define the earliest critical step as  
\begin{equation}
    t^\ast = \arg\min_{t} \{\, y(\tau^{(t \to \hat{a}_t)})=1 \,\},
\end{equation}
where $\tau^{(t \to \hat{a}_t)}$ denotes a trajectory with corrected action $\hat{a}_t$. By linking $\hat{a}_t$ to the \AET{} error label $e_t^m$, \ModelName{} isolates not just \emph{when} the trajectory first goes wrong, but also \emph{why} (e.g., misrecall in memory, infeasible plan, or malformed action).  

\paragraph{Stage 3: Iterative Debugging.}  
For the detected error $e_{t^\ast}$, \ModelName{} generates targeted feedback
\begin{equation}
    \phi_{t^\ast} = \psi(s_{t^\ast},a_{t^\ast},e_{t^\ast}),
\end{equation}
and performs a re-rollout:
\begin{equation}
    \tau^{(k+1)} = \text{ReRollout}(\tau^{(k)},\phi_{t^\ast}^{(k)}), \quad k=1,\dots,B.
\end{equation}
The process repeats until $y(\tau^{(k+1)})=1$ or budget $B$ is reached. Theok feedback is conditioned on \AET{} categories, re-rollouts are interpretable and targeted rather than ad hoc.  




==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

